Contrastive Weight Regularization for Large Minibatch SGD

The minibatch stochastic gradient descent method (SGD) is widely applied in deep learning due to its efficiency and scalability that enable training deep networks with a large volume of data. Particularly in the distributed setting, SGD is usually applied with large batch size. However, as opposed to small-batch SGD, neural network models trained with large-batch SGD can hardly generalize well, i.e., the validation accuracy is low. In this work, we introduce a novel regularization technique, namely distinctive regularization (DReg), which replicates a certain layer of the deep network and encourages the parameters of both layers to be diverse. The DReg technique introduces very little computation overhead. Moreover, we empirically show that optimizing the neural network with DReg using large-batch SGD achieves a significant boost in the convergence and improved generalization performance. We also demonstrate that DReg can boost the convergence of large-batch SGD with momentum. We believe that DReg can be used as a simple regularization trick to accelerate large-batch training in deep learning.

==> related_work_v0.tex <==
\section{Background}

\paragraph{Minibatch SGD} Minibatch SGD is the dominate algorithm for optimizing deep neural networks (DNNs) derived from SGD. Let $f(\cdot; W)$ be a DNN model parameterized by $W$, which is trained on a finite training set $X$ of $M$ samples. Train a network using SGD is to minimize the loss function $\mathcal{L}(W)$,
\begin{equation}
\scriptsize
    \mathcal{L}(W) = \frac{1}{M}\sum_{x \in X}l(x, W),
\end{equation}
where $\mathcal{L}(W)$ is the average of the loss $l$ of every training data in the training set.
Instead of updating the parameters $W$ based on a single training example, minibatch SGD \cite{minibatchSGD} updates the $W$ using the gradients obtained from a minibatch $\mathcal{B}$ of $M$ training examples.
The weight update rule of minibatch SGD can be written as follows:
\begin{equation}
\scriptsize
    \label{eq:minibatch}
    W_{(t+1)} = W_{(t)} - \eta \frac{1}{m}\sum_{x \in \mathcal{B}}\nabla l(x, W_{(t)}),
\end{equation}
where $\eta$ is the stepsize (i.e., learning rate) and $t$ is the index of the training iteration.
Moreover, momentum SGD \cite{momentumSGD} is a widely-adopted method to accelerate the vanilla minibatch SGD in Equation~\ref{eq:minibatch}.
To update the parameters with less noisy gradients, a momentum is defined as a moving average of the minibatch gradients and used to update the parameters of the form:
\begin{equation}
\scriptsize
\label{eq:momentum}
\begin{split}
    v_{(t+1)} &= \beta v_{(t)} + \frac{1}{m}\sum_{x \in \mathcal{B}}\nabla l(x, W_{(t)}) \\
    W_{(t+1)} &= W_{(t)} - \eta v_{(t+1)}
\end{split}
\end{equation}
Here, $\beta$ denotes the momentum decaying factor and $v$ is the update tensor.
The momentum SGD can be considered as the state-of-the-art optimization algorithm for DNNs.
The proposed distinctive regularization method can speedup the convergence and improve the generalization of DNNs trained using both the vanilla and momentum SGD.

\paragraph{Large Minibatch SGD} Many recent works \cite{fb_largebatch, google_largebatch} propose to scale up the training of large DNN models by using a very large minibatch size $\mathcal{B}$. The large batch SGD is enabled by distributing the minibatch over $K$ devices, where a minibatch of $\frac{\mathcal{B}}{K}$ training examples is trained on each device. Therefore, the overall batch size $\mathcal{B}$ can be scaled up linearly with the number of devices $K$. However, training with a large batch size typically increases the generalization gap (i.e., a degraded test accuracy) \cite{largebatch1, largebatch2, largebatch3}. To the best of our knowledge, there are a few attempts to close the generalization gap in literature. 
\citet{fb_largebatch} propose a learning rate warm up scheme, which increases the learning rate linearly with the training iterations. 
\citet{lars} propose to scale the learning rate of each layer to enable a large batch size.
\citet{anisotropic_noise, wen2019empirical} propose to inject anisotropic and empirical noise to lower the generalization gap. However, these noise injecting methods are usually very compute intensive. As the proposed distinctive regularization is orthogonal to the aforementioned techniques, we believe that the distinctive regularization can be used together to further minimize the test accuracy degradation caused by a large batch size.

\paragraph{Regularization}
Adding regularizer to the total loss can help to promote a specific structure on the solution. For example, $\ell_2$ regularization is used to control the weight norm and improve generalization \cite{Krogh1991}, $\ell_1$ and group $\ell_1$ regularization impose  (group) sparsity structure on the model parameters \cite{Tibshirani2011,Simon2013}, and nuclear norm regularization constraints the high dimensional parameters within a low dimensional subspace \cite{candes2012,Toh2010}. Other approaches regularize the algorithm update rules, e.g., the cubic regularization algorithm \cite{nesterov2006,zhou2018,wang19d}. All these conventional regularization approaches do not change the model structure. On the other hand, multi-task learning shares a subset of model parameters for different tasks and
can be viewed as a type of model regularization \cite{Caruana1993,duong-etal-2015}. Compare to the soft multi-task learning approach \cite{duong-etal-2015} which penalizes the distance among these models and encourage them to be similar, our distinctive regularization promotes a large distance between the models and desires diverse models.



%Reference uses \cite{Alizadeh:tcad10}.
